Multilateral Micro-Monitoring for Internet Streaming

Video streaming is dominating the Internet. To compete with the performance of traditional cable and satellite options, content providers outsource the content delivery to third-party content distribution networks and brokers. However, no existing monitoring mechanism offers a multilateral view of a streaming service's performance. In other words, no auditing mechanism reflects the mutual agreement of content providers, content distributors and end-users alike about how well, or not, a service performs. In this paper, we present UgoVor, a system for monitoring multilateral streaming contracts, that is enforceable descriptions of mutual agreements among content providers, content distributors and end-users. Our key insight is that real-time multilateral micro-monitoring -- capable of accounting for every re-buffering event and the resolution of every video chunk in a stream -- is not only feasible, but an Internet-scalable task. To demonstrate this claim we evaluate UgoVor in the context of a 10-month long experiment, corresponding to over 25 years of streaming data, including over 430,000 streaming sessions with clients from over 1,300 unique ASes. Our measurements confirm that UgoVor can provide an accurate distributed performance consensus for Internet streaming, and can help radically advance existing performance-agnostic pricing model towards novel and transparent pay-what-you-experience ones.

==> section/ethics.tex <==

This work does not raise any ethical issues. In particular, the streaming data set we were provided with includes no
personally-identifiable information, and no user-identifiable or traceable information. For example, if the same user utilized the Live TV streaming
twice, this would show up as two independent users in the trace. The trace does provide AS-level information, which helped us
detect mobile vs. cable network operators. However, we anonymized this information in the paper. 



==> section/implementation.tex <==
The client has a browser plugin that detects any changes in QoE by making API calls exposed to us by the HTML5 video element. The plugin also connects to a native python application that handles explicit communication with the auditor on a specially known port. The server monitor is implemented as a python process for each contracted session. The server monitor also maintains explicit communication with the enforcer. Additionally, the server monitor builds its view with the information that comes from egress nodes serving the client with media streams. All communication with the enforcer from the client monitor as well as the server monitor are through session-long TCP connections. The auditor is also implemented in python as a multithreaded TCP server.  


==> section/motivation.tex <==
Do we need to explain why micro-auditing of QoE is necessary in real time? 
People pay flat-prices but get a varied level of quality that may often not reflect the best effort of a content provider. People should have more say in what they want to consume at what price?

Are examples such as the Facebook Advertizer issue where Advertizers could not verify in real time video metrics apt here? We could potentially say that such pitfalls for third parties can be overcome if they have a hook into the entire streaming process in real time without having to rely on any one end-point.

